Reasoning on $\textit{DL-Lite}_{\cal R}$ with Defeasibility in ASP

Reasoning on defeasible knowledge is a topic of interest in the area of description logics, as it is related to the need of representing exceptional instances in knowledge bases. In this direction, in our previous works we presented a framework for representing (contextualized) OWL RL knowledge bases with a notion of justified exceptions on defeasible axioms: reasoning in such framework is realized by a translation into ASP programs. The resulting reasoning process for OWL RL, however, introduces a complex encoding in order to capture reasoning on the negative information needed for reasoning on exceptions. In this paper, we apply the justified exception approach to knowledge bases in $\textit{DL-Lite}_{\cal R}$, i.e., the language underlying OWL QL. We provide a definition for $\textit{DL-Lite}_{\cal R}$ knowledge bases with defeasible axioms and study their semantic and computational properties. In particular, we study the effects of exceptions over unnamed individuals. The limited form of $\textit{DL-Lite}_{\cal R}$ axioms allows us to formulate a simpler ASP encoding, where reasoning on negative information is managed by direct rules. The resulting materialization method gives rise to a complete reasoning procedure for instance checking in $\textit{DL-Lite}_{\cal R}$ with defeasible axioms. Under consideration in Theory and Practice of Logic Programming (TPLP).

==> sec/dkb-model-checking.tex <==

%\section{Intractability of DKB-Model Checking}    
    
\begin{proposition}    
Deciding whether a given CAS-model $\IC_{\CAS}$ of a DKB
$\DKB$ is justified is \conp-hard.
\end{proposition}

\begin{proof}
We show this by a reduction from deciding whether a directed graph
$G=(V,E)$ has some Hamiltonian path starting at a given node $s$, i.e.,
a path that visits all nodes but no one twice. 

We construct $\DKB$ as follows. Each vertex $v_i$ in
$V=\{v_1,\ldots,v_n\}$ is an individual, and we take distinct
individuals $w_0,\ldots,w_n$. The idea is to add to $G$ the path 
$\pi = w_0,w_1,w_2,\ldots,w_n$ and an edge $(w_0,s)$. We
use roles $R_i$, $i=1,\ldots,n$ to form a role chain 
$R_1(u_0,u_1)$, $R_2(u_1,u_2)$, \ldots, $R_n(u_{n-1},u_n)$ starting at 
$u_0=w_0$, where all $u_i$, $i>0$ must be nodes $v_j$ or
$w_j$. Furthermore, we shall enforce that all the $u_i$ must be
distinct.  There is one such role chain if $u_i = w_i$, for all
$i=0,\ldots,n$ leading to $w_n$. At this node, we shall make an
exception to a default, which can be only justified by an incoming
$R_n$ edge. Furthermore, the justification will require that in each
model there is an incoming $R_n$ edge; this will only be possible if
the input graph $G$ has no Hamiltonian path.

To realize this, we use the following axioms and defeasiable axioms under UNA: 

\begin{enumerate}
  \item  $\exists R_1(w_0)$,\ $D(w_0)$,  $D(v_i)$, $D(w_i)$,
        $i=1,\ldots, n$ 
  \item  $\neg R(u,u')$ where  $u,u'$ are from $U = \{ w_0,w_1,v_1,\ldots,
        w_n,v_n\}$ and $(u,u') \notin E' = E \cup \{ (w_0,s) \} \cup
        \{ (w_{i-1},w_i) \mid i=1,\ldots,n\}$

 \item $\exists R^-_i \isa \non\exists R^-_j $, for all $i\neq j$

  \item $\exists R_i \isa \non\exists R_j $, for all $i\neq j$  
  
%  \item $\exists R_i \isa \exists R^-_{i-1} $, for all $i > 0$
  
  \item $\exists R^-_{i-1} \isa \exists R_i$, for all $i > 0$

 \item $R_i \isa R$, for $i=1,\ldots n$
 
 \item $\exists R^- \isa D$,  $\exists R \isa D$, 
 
 \item  $\default(D \isa \bot)$ and $\default(\non R^-_n(w_n))$
\end{enumerate}

$D$ is a domain predicate, for which exceptions will be made on for
the individuals in $\DKB$. This will by 2) and 7) enforce that an $R(u,u')$
edges, and thus by 6) also an $R_i(u,u')$ edge can only exist if
$(u,u')$ is in $E'$. The axioms in 3) - 5) ensure that if a node $u$ has
an incoming $R_i$ edge, then it can only have incoming $R_i$ edges and
it must have an outgoing $R_{i+1}$  edges and only such among the
$R_j$, if $i<n$, The will enforces that a
partially built chain $R_1(u_0,u_1)$, \ldots, $R_i(u_{i-1},u_i)$ in
which all nodes are distinct will be continued with an edge
$R_{i+1}(u_i,u_{i+1})$ to a node $u_i$ distinct from
$u_0,\ldots,u_i$. In particular, a complete such chain that has
$u_0=w_0$, $u_1=s$ must contain a Hamiltonian path $u_1,\ldots,u_n$ in $G$

Formally, we let $\Ical$ be induced by $R_1(w_0,w_1)$, $R_2(w_1,w_2)$,
\ldots, $R_n(w_{n-1},w_n)$ (the least model)
where $\casmap = \{ \stru{D\isa \bot, u} \mid u\in U\} \cup \{
\stru{\neg\exists R^-_nn(w_n),()}\}$. Then it holds that $\IC_{\CAS} =
\stru{\Ical,\casmap}$ is a CAS-model of $\DKB$.
                        
It can be shown that in every (NI-congruent) CAS-model
$\IC'_{\CAS} = \stru{\Ical',\casmap}$, some chain $R_1(u_0,u_1),$
$\ldots,$ $R_n(u_{n-1},u_n)$, 
where $u_0=w_0$ and all $u_i$ are distinct exists. Furthermore, 
$R_1(w_0,w_1)$, $R_2(w_1,w_2),$ \ldots, $R_n(w_{n-1},w_n)$ is the only
such chain iff in $G$ no Hamiltonian path starting at $s$ exists. 

Thus, if no alternative chain exists, then in every model
$\IC'_{\CAS}$ as above the atom $R_n(w_{n-1},w_n)$, and thus $\exists
R_n^-(w_n)$ is true; this $\IC_{\CAS}$ is justified.
Conversely, if $\IC_{\CAS}$ is justified, 
then in every $\IC'_{\CAS}$ model as above the atom $\exists R^n(w_n)$ must be
true. This means that no alternative chain exists, as otherwise we
could make $R_1(w_0,w_1)$, $R_2(w_1,w_2),\ldots, R_n(w_{n-1},w_n)$ all
false in that model. This proves the result.
\end{proof}

As consequence of the construction, also deciding whether a partial CAS-model $\IC_{\CAS}
= \stru{\Ical,\casmap}$ where $\Ical$ that is merely described on the ABox
individuals can be extended to some DKB model $\IC'_{\CAS} =
\stru{\Ical',\casmap}$ is \conp-hard. 

%Furthermore, we note that the DKB $\DKB$ constructed in the proof is
%acyclic and moreover $O(n)$-de safe, i.e., only a linear number of
%Skolem terms can be derived that feed into clashing sets.

